Production and validation of scintillating structural components from low-background Poly(ethylene naphthalate)

Poly Ethylene Naphthalate (PEN) is an industrial polymer plastic which is investigated as a low background, transparent, scintillating and wavelength shifting structural material. PEN scintillates in the blue region and has excellent mechanical properties both at room and cryogenic temperatures. Thus, it is an ideal candidate for active structural components in experiments for the search of rare events like neutrinoless double-beta decay or dark matter recoils. Such optically active structures improve the identification and rejection efficiency of background events, like this improving the sensitivity of experiments. This paper reports on the production of radiopure and transparent PEN plates These structures can be used to mount germanium detectors operating in cryogenic liquids (LAr, LN). Thus, as first application PEN holders will be used to mount the Ge detectors in the LEGEND-200 experiment. The whole process from cleaning the raw material to testing the PEN active components under final operational conditions is reported.

==> sections/05-scintillation.tex <==
\section{Scintillation output}\label{sec:scintillation} 
Besides the excellent mechanical properties of PEN at cryogenic temperatures \cite{Efremenko:2019xbs} and the very good radiopurity achieved during this first production for \textsc{Legend}-$200$, the wavelength shifting capabilities and scintillation properties provide major advantages. These optical properties are very important and, among others, include the light output and the attenuation length. Custom-made scintillators as described in this paper, could have different properties depending on various settings in the production. In order to classify and compare production batches, a test station was designed at the Max Planck Institute for Physics in Munich, Germany. This setup is composed of five square-shaped PMTs with an active area of $23\times 23$\,mm$^2$ (HAMAMATSU H$11934$-$300$). Four of them surround PEN samples of $30\times30\times1.5$\,mm$^3$ and the fifth is placed beneath it. This configuration was chosen in order to cover as much surface of the PEN samples as possible. The coverage is estimated to be about $34$\,\% due to the active area of the PMTs. Optical grease (EJ-$550$) is used to improve the light guiding from the scintillator to the photo sensors. Finally, a $^{207}$Bi\,source was chosen due to its emission of MeV scale electrons. A PTFE collimator is placed between the source and the samples. This ensemble was placed on a 3D printed holder. A trigger system to select electrons from $^{207}$Bi\,source was also developed. A more detailed description of the setup and analysis of the optical properties of this \textsc{Legend}-$200$ PEN production will be presented soon in a follow-up paper. The triggered events were recorded using a Struck SIS-$3316$ digitizer with $250$\,MHz sampling rate and $14$\,bit resolution. Here, the waveforms of all six PMTs are stored for offline analysis.

Before data taking starts, a short calibration run is performed for all PMTs. Here, a pulsed UV LED is used and was illuminated at low intensity to produce just enough light to see the $1$\,photo-electron (p.e.) peak in the spectrum. More details regarding the calibration will be reported in our follow-up paper. The sum of the signals from the five PMTs coupled to the sample then gives the total charge in photo-electrons, which is shown in Figure\,\ref{fig:side_pmts_total}. The dominant peak in the Bi spectrum corresponding to around $950$\,keV can be clearly recognized and yields around $530$\,photons. This result validate the scintillation properties of this \textsc{Legend}-$200$ production run.

%\begin{figure}
%    \centering
    %\includegraphics[width=0.4\textwidth]{figures/6pmt_MC.png}
%\includegraphics[width=0.55\textwidth]{figures/06-spe.pdf}
 %   \caption{Left: Schematic of the setup. CREATE NEW SCHEMATIC! Right: Single photo-electron calibration of one of the six PMTs in the setup. A pulsed UV-LED was used as light source.}
 %   \label{fig:setup}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Light_output_PEN.pdf}
    \caption{Light output for PEN samples excited with a $^{207}$Bi source. The total charge corresponds to the sum of the charges in all five PMTs coupled to the Sample. \textbf{here we need to decide if we put this figure or another one including SP32 or EJ-200 for comparison, knowing that a detailed optical properties paper is coming.}}
    \label{fig:side_pmts_total}
\end{figure}


